Mamba in Speech: Towards an Alternative to Self-Attention

Transformer and its derivatives have achieved success in diverse tasks across computer vision, natural language processing, and speech processing. To reduce the complexity of computations within the multi-head self-attention mechanism in Transformer, Selective State Space Models (i.e., Mamba) were proposed as an alternative. Mamba exhibited its effectiveness in natural language processing and computer vision tasks, but its superiority has rarely been investigated in speech signal processing. This paper explores solutions for applying Mamba to speech processing by discussing two typical speech processing tasks: speech recognition, which requires semantic and sequential information, and speech enhancement, which focuses primarily on sequential patterns. The experimental results confirm that bidirectional Mamba (BiMamba) consistently outperforms vanilla Mamba, highlighting the advantages of a bidirectional design for speech processing. Moreover, experiments demonstrate the effectiveness of BiMamba as an alternative to the self-attention module in the Transformer model and its derivates, particularly for the semantic-aware task. The crucial technologies for transferring Mamba to speech are then summarized in ablation studies and the discussion section, offering insights for extending this research to a broader scope of tasks.

==> ASR_table/ASR_Main.tex <==
\begin{table}[t] 
\centering
\scriptsize
\def\arraystretch{1.25}
\setlength{\tabcolsep}{1pt}
  \setlength{\abovetopsep}{0pt}
  \setlength\belowbottomsep{0pt} 
  \setlength\aboverulesep{0pt} 
  \setlength\belowrulesep{0pt}
\caption{ASR results for the different datasets without language model in WER/MER (\%). ``ESPnet'' means the best result reported by ESPnet official or other paper experimented with ESPnet, where the SEAME and ASRU results come from~\cite{liu23_icassp,liu2024enhancing, liu2024aligning}.} 
\resizebox{\columnwidth}{!}{
\begin{tabular}{@{}l@{\hspace{4pt}}ccccccccc@{}}
\toprule[1.25pt]
\textbf{Method} &  & \multicolumn{2}{c}{LibriSpeech-100} & \multicolumn{2}{c}{LibriSpeech-960} & \multicolumn{2}{c}{SEAME} & \multicolumn{2}{c}{ASRU}\\
\cmidrule(lr){3-4} \cmidrule(lr){5-6} \cmidrule(lr){7-8} \cmidrule(lr){9-10} 
& & dev & test & dev & test & man & sge  & dev & test \\
\midrule
\textit{ESPnet} & & & & & & & & & \\
\quad Conformer &  & 6.3 & 6.5 & 2.1 & 2.4 & 16.6 & 23.3 & - & 12.2 \\
\quad Branchformer &  & 6.1 & 6.3 & 2.2 & 2.4 & - & - & - & - \\
\hline
\hline
\multicolumn{3}{l}{\textit{Reproduced Results}}  \\
\quad Branchformer &  & 6.3 & 6.4 & 2.2 & 2.4 & \textbf{16.3} & \textbf{23.2} & 12.5 & 11.8 \\
\hdashline
\quad Mamba &  & 40.8 & 40 & 21.8 &22.3 &44.5 &55.3 &38.0 &36.3 \\
\quad  InnBiMamba  &  & 39.6 & 38.2 & 21.8 &22.5 & 44.3 & 55.4 &38.4 &37.9 \\
\quad ExtBiMamba  &  & 38.5 & 37.7 & 21.6 &22.1 & 44.4 & 55.2 &38.2 &36.8 \\
\hdashline
\quad Transformer &  & 8.0 & 8.4 & 2.8 & 3.2 & 17.7 & 24.5 & 13.7 & 13.1 \\
\quad $-$ MHSA $+$ Mamba &  & 10.9 & 11.2& 3.2 &3.5  & 20.7 &29.5 &24.2 &23.1 \\
\quad $-$ MHSA $+$  InnBiMamba  &  & 8.8 & 9.4 & 2.5 & 3.0 & 18.4 &26.0 &20.2 & 19.5 \\
\quad $-$ MHSA $+$ ExtBiMamba  &  & 8.4 & 8.7 & 2.5 & 2.8 & 17.2 &24.3 &18.7 & 18.0 \\
\hdashline
\quad Conformer &  & 6.3 & 6.5 & 2.3 & 2.6 & 16.9 & 23.6 & 12.8 & 12.2 \\
\quad $-$ MHSA $+$ Mamba &  & 6.6 & 6.9 & 2.6 & 2.9 & 17.7 & 24.9 & 13.5 & 12.9\\
\quad $-$ MHSA $+$  InnBiMamba  &  & 6.0 & 6.4 & 2.1 & 2.3 & 17.1 &23.8 &12.7 & 12.2 \\
\quad $-$ MHSA $+$ ExtBiMamba  &  & \textbf{5.9} & \textbf{6.0} & \textbf{2.0} & \textbf{2.3} & 16.6 & 23.4 & \textbf{12.3} & \textbf{11.5}\\
\toprule[1.25pt]
\end{tabular}
}
% \vspace{-1.0em}
\label{ASR Main Result}
\end{table}


==> ASR_table/Ablation_Study_on_liber100.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1pt} % 减少列间距
\caption{Ablation Study on LibriSpeech100 for \textcolor{black}{ConExtBiMamba} by employing WER (\%)}
\resizebox{\columnwidth}{!}{ % 缩小表格以适应单列
\begin{tabular}{lcccc}
\toprule[1.0pt]
\textcolor{blue}{\textbf{Model}} & \textbf{dev\textdownarrow} & \textbf{dev other\textdownarrow} & \textbf{test\textdownarrow} & \textbf{test other\textdownarrow} \\
\midrule
ConvExtBiMamba with Gaussian Noise & 5.9 & 17.1 & 6.0 & 17.3 \\
\quad $\rightarrow$ $d_{\text{state}}=32$ & 5.9 & 17.1 & 6.0 & 17.3 \\
\quad $\rightarrow$ $d_{\text{conv}}=2$ & 6.0 & 17.1 & 6.2 & 17.3 \\
\quad $\rightarrow$ $E=4$ & 5.9 & 17.1 & 6.0 & 17.3 \\
\quad $\rightarrow$ Random Noise A matrix & 6.0 & 17.2 & 6.2 & 17.4 \\
\quad $\rightarrow$ default A matrix & 6.1 & 17.2 & 6.2 & 17.5 \\
\quad \textcolor{blue}{$\rightarrow$ complex-valued A matrix} & \textcolor{blue}{6.0} & \textcolor{blue}{17.2} & \textcolor{blue}{6.2} & \textcolor{blue}{17.3} \\
\toprule[1.0pt]
\end{tabular}
}
\label{Ablation Study on liber100}
\end{table}


==> ASR_table/Ablation_Study_on_liber100_Conv-BiMamba.tex <==
\begin{table}[t]
\centering
% \scriptsize
\small
\setlength{\tabcolsep}{1pt} % 减少列间距
\caption{Ablation Studies for \textcolor{black}{ConExtBiMamba} on LibriSpeech100.}
% \resizebox{\columnwidth}{!}{ % 缩小表格以适应单列
\begin{tabular}{lcccc}
\toprule[1.0pt]
\textcolor{blue}{\textbf{Method}} & \textbf{dev\textdownarrow} & \textbf{dev other\textdownarrow} & \textbf{test\textdownarrow} & \textbf{test other\textdownarrow} \\
\midrule
\textcolor{black}{ConExtBiMamba} & 5.9 & 17.1 & 6.0 & 17.3 \\
\quad $-$ Macaron & 6.1 & 17.7 & 6.3 & 17.9 \\
\quad $-$ Swish & 6.2 & 17.7 & 6.4 & 18.1 \\
\quad $-$ Dropout & 6.0 & 17.1 & 6.0 & 17.4 \\
\quad $+$ Positional Encoding & 6.0 & 17.1 & 6.0 & 17.3 \\
\toprule[1.0pt]
\end{tabular}
% }
\label{Ablation Study on liber100 Conv-BiMamba}
\end{table}


==> ASR_table/BiMambaV1_vs_BiMambaV2_in_seame_and_asru.tex <==
\begin{table}[t]
\centering
\scriptsize
\setlength{\tabcolsep}{1pt} % 减少列间距
\caption{InnBiMamba \textcolor{blue}{vs.} ExtBiMamba: MER Results (\%) on ASRU and SEAME. Left results are from ASRU, right results are from SEAME.}
\resizebox{\columnwidth}{!}{ % 缩小表格以适应单列
\begin{tabular}{lcccccc}
\toprule[1.25pt]
\textbf{Method} & \textbf{Params (M)} & \textbf{dev} & \textbf{test} & \textbf{Params (M)} & \textbf{man} & \textbf{sge} \\
\midrule
Transformer & 30.86 & 13.7 & 13.1 & 29.86 & 17.7 & 24.5   \\
\quad $-$ MHSA $+$ InnBiMamba & 34.80 & 20.2 & 19.5  & 33.81 & 18.4 & 26.0 \\
\quad $-$ MHSA $+$ ExtBiMamba  & 44.24 & 18.7 & 18 & 43.25 & 17.2 & 24.3 \\
\hdashline
Conformer & 48.27 & 12.8 & 12.2 & 47.27 & 16.9 & 23.6   \\
\quad $-$ MHSA $+$ InnBiMamba & 50.10 & 12.7 & 12.2 & 49.11 & 17.1 & 23.8\\
\quad $-$ MHSA $+$ ExtBiMamba & 56.40 & \textbf{12.3} & \textbf{11.5} & 55.40 & \textbf{16.6} & \textbf{23.4}  \\
\toprule[1.25pt]
\end{tabular}
}
\label{Bidirectional V1 Vs Bidirectional V2 in ASRU and SEAME}
\end{table}


==> ASR_table/complete_result_liberspeech.tex <==
\begin{table}[t]
\centering
\scriptsize
\def\arraystretch{1.25}
\setlength{\tabcolsep}{2pt} % 减少列间距
\setlength{\abovetopsep}{0pt}
\setlength\belowbottomsep{0pt} 
\setlength\aboverulesep{0pt} 
\setlength\belowrulesep{0pt}
\caption{WER results on LibriSpeech (without external language model) across various parameter counts and frameworks.}
\resizebox{\columnwidth}{!}{ % 缩小表格以适应单列
\begin{tabular}{lccccc}
\toprule[1.25pt]
\textbf{Method} & \textbf{Params (M)} & \textbf{dev} & \textbf{dev other} & \textbf{test} & \textbf{test other} \\
\midrule
\multicolumn{4}{l}{\textit{LibriSpeech100}} \\
Transformer & 29.38 & 8.0 & 20.0 & 8.4 & 20.2 \\
\quad $-$ MHSA $+$ InnBiMamba & 33.32 & 8.8 & 23.3 & 9.4 & 23.6 \\
\quad $-$ MHSA $+$ ExtBiMamba & 40.42 & 8.4 & 22.4 & 8.7 & 23.1 \\
\hdashline
Conformer Large & 42.17 & 6.2 & 17.4 & 6.4 & 17.3 \\
Conformer & 34.23 & 6.3 & 17.4 & 6.5 & 17.3 \\
\quad $-$ MHSA $+$ InnBiMamba & 36.89 & 6.0 & 17.4 & 6.4 & 17.6 \\
\quad $-$ MHSA $+$ InnBiMamba Large & 49.90 & 6.1 & 17.3 & 6.3 & 17.3 \\
\quad $-$ MHSA $+$ ExtBiMamba & 41.59 & \textbf{5.9} & \textbf{17.1} & \textbf{6.0} & \textbf{17.2} \\
\midrule
\multicolumn{4}{l}{\textit{LibriSpeech960}} \\
Transformer & 99.36 & 2.8 & 7.6 & 3.2 & 7.5 \\
\quad $-$ MHSA $+$ InnBiMamba & 103.35 & 2.5 & 7.4 & 3.0 & 7.3 \\
\quad $-$ MHSA $+$ ExtBiMamba & 110.04 & 2.5 & 6.9 & 2.8 & 6.9 \\
\hdashline
Conformer & 116.15 & 2.3 & 5.5 & 2.6 & 5.6 \\
\quad $-$ MHSA $+$ InnBiMamba & 118.81 & 2.1 & 5.6 & 2.4 & 5.5 \\
\quad $-$ MHSA $+$ ExtBiMamba & 123.51 & \textbf{2.0} & \textbf{5.4} & \textbf{2.3} & \textbf{5.4} \\
\toprule[1.25pt]
\end{tabular}
}
\label{Completed Result on liber960}
\vspace{-1.3em}
\end{table}


==> ASR_table/mamba_size_table.tex <==
\begin{table}[t]
\centering
\scriptsize
\def\arraystretch{1.12}
\setlength{\tabcolsep}{1pt}
\setlength{\abovetopsep}{0pt}
\setlength\belowbottomsep{0pt} 
\setlength\aboverulesep{0pt} 
\setlength\belowrulesep{0pt}
\caption{WER/MER results (\%) for LibriSpeech100 and SEAME: the left part displays results from LibriSpeech100, while the right part shows results from SEAME.}
\resizebox{\columnwidth}{!}{
\begin{tabular}{lccc|cccc}
\toprule[1.25pt]
\textbf{Method} & \textbf{\#Params (M)} & \textbf{dev } & \textbf{test} & \textbf{\#Params (M)} & \textbf{man } & \textbf{sge}\\
\midrule
Conformer & 34.23 & 6.3 & 6.5 & 47.27 & 16.9 & 23.6 \\
Transformer & 29.38 & 8.0 & 8.4 & 29.38 & 17.7 & 24.5 \\
\midrule
\multicolumn{4}{l}{\textit{Mamba-based Models}} \\
Mamba & 20.41 & 40.8 & 40 & 20.41 & 44.5 & 55.3 \\
Mamba Large & 32.52 & 38.8 & 39.2 & 28.78 & 45.5 & 55 \\
\hdashline
ExtBiMamba & 25.79 & 38.5  & 37.7 & 25.79 & 44.4  & 55.2 \\
ExtBiMamba Large & 33.52 & 37.8 & 37.2 & 33.52 & 43.6 & 54.3 \\
\toprule[1.25pt]
\end{tabular}
}
\label{Small Mamba VS large Mamba on Liberspeech 100}
\end{table}


==> New_asr_table/information_plane.tex <==
\begin{figure}[!t]
    \centering
    \begin{subfigure}[b]{0.48\columnwidth} % 调整子图宽度为单列的一半
        \includegraphics[width=\textwidth]{New_asr_table/BiMamba.pdf}
        \caption{IP for BiMamba}
        \label{IP_BiMamba}
    \end{subfigure}
    \hfill
    \begin{subfigure}[b]{0.48\columnwidth} % 调整子图宽度为单列的一半
        \includegraphics[width=\textwidth]{New_asr_table/ConExtBimamba.pdf}
        \caption{IP for ConExtBiMamba}
        \label{IP_ConExtBiMamba}
    \end{subfigure}
     \caption{\textcolor{blue}{Information Plane for Bimamba and ConExtBimamba in ASR Task}}
    \label{fig:information_plane}
\end{figure}

==> SE_table/ConvMamba.tex <==
\begin{table}[!h]
    \centering
    \scriptsize
    \def\arraystretch{1.30}
    \setlength{\tabcolsep}{1pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
    \caption{Evaluation results for replacing the MHSA with Mamba/BiMamba layer in Conformer network, across causal and noncausal configurations.}
    \label{tab:conmamba}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lrccccccc@{}}
        \toprule[1.0pt]
        \multirow{2}{*}{\textbf{Model}} & \multirow{2}{*}{\textbf{\#Para.}} & \multirow{2}{*}{\textbf{Cau.}} & \multicolumn{6}{c}{\textbf{Metrics}}\\  
        \cline{4-9}
        & & & NB-PESQ & WB-PESQ & ESTOI & CSIG & CBAK & COVL \\  
        \midrule
        Noisy  & -- & -- & \textcolor{black}{1.88} & \textcolor{black}{1.24} & \textcolor{black}{56.12} & \textcolor{black}{2.26} & \textcolor{black}{1.80} & \textcolor{black}{1.67} \\
        Conformer-4 &  6.22M  &  \ding{52}   & \textcolor{black}{2.67} & \textcolor{black}{1.94} & \textcolor{black}{72.78} & \textcolor{black}{\bf 3.29} & \textcolor{black}{2.45} & \textcolor{black}{2.58}  \\
        \, \textcolor{blue}{MHSA$\rightarrow$Mamba} &  6.92M & \ding{52}   & \textcolor{black}{\bf 2.69} & \textcolor{black}{\bf 1.95} & \textcolor{black}{\bf 73.27} & \textcolor{black}{\bf 3.29} & \textcolor{black}{\bf 2.48} & \textcolor{black}{\bf 2.59}  \\
        \hdashline
        Conformer-4 & 6.22M  & \ding{55} & \textcolor{black}{2.88} & \textcolor{black}{2.17} & \textcolor{black}{76.68} & \textcolor{black}{3.51} & \textcolor{black}{2.61} & \textcolor{black}{2.82}  \\
        \, \textcolor{blue}{MHSA$\rightarrow$InnBiMamba}  &  7.10M  & \ding{55} & 2.89 & 2.17 & 77.40 & 3.51 & 2.62 & 2.81  \\
        \, \textcolor{blue}{MHSA$\rightarrow$ExtBiMamba}  &  8.67M  & \ding{55} & \bf 2.92 & \bf 2.20 & \bf 77.74 & \bf 3.57 & \bf 2.64 & \bf 2.88  \\
        \hline
        \hline
        Conformer-6 &  9.26M  &  \ding{52}   & \textcolor{black}{2.68} & \textcolor{black}{1.94} & \textcolor{black}{73.41} & \textcolor{black}{3.30} & \textcolor{black}{2.46} & \textcolor{black}{2.59}  \\
        \, \textcolor{blue}{MHSA $\rightarrow$Mamba} & 10.32M  &  \ding{52}   & \textcolor{black}{\bf 2.71} & \textcolor{black}{\bf 1.95} & \textcolor{black}{\bf 73.69} & \textcolor{black}{\bf 3.34} & \textcolor{black}{\bf 2.49} & \textcolor{black}{\bf 2.62}  \\
        \hdashline
        Conformer-6 & 9.26M  & \ding{55} & \textcolor{black}{2.91} & \textcolor{black}{2.20} & \textcolor{black}{77.56} & \textcolor{black}{3.54} & \textcolor{black}{2.62} & \textcolor{black}{2.84}  \\
        \, \textcolor{blue}{MHSA$\rightarrow$InnBiMamba} & 10.59M  & \ding{55} & 2.92 & 2.19 & 77.85 & 3.52 & 2.64 & 2.83 \\
        \, \textcolor{blue}{MHSA$\rightarrow$ExtBiMamba} & 12.94M  & \ding{55} & \bf 2.93 & \bf 2.23 & \bf 78.21 & \bf 3.60 & \bf 2.65 & \bf 2.89 \\
        \toprule[1.0pt]
    \end{tabular}}
    % \vspace{-0.5em}
\end{table}


==> SE_table/Mamba_Conformer_SE.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \def\arraystretch{1.25}
    \setlength{\tabcolsep}{1pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
    \caption{Speech enhancement performance comparisons of Conformer and Mamba network architectures in N-PESQ, W-PESQ, ESTOI (\%), CSIG, CBAK, and COVL, across causal and noncausal configurations. The Conformer models with $4$ and $6$ Conformer layers are denoted as Conformer-4 and Conformer-6, respectively.}
    \label{tab:conformer_mamba}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lcccccccc@{}}
        \toprule[1.0pt]
        \multirow{2}{*}{\textbf{Method}} & \multirow{2}{*}{\textbf{\#Para.}} & \multirow{2}{*}{\textbf{Cau.}} & \multicolumn{6}{c}{\textbf{Metrics}}\\  
        \cline{4-9}
        & & & N-PESQ$\uparrow$ & W-PESQ$\uparrow$ & ESTOI$\uparrow$ & CSIG$\uparrow$ & CBAK$\uparrow$ & COVL$\uparrow$ \\  
        \midrule
        Noisy  & -- & -- & \textcolor{black}{1.88} & \textcolor{black}{1.24} & \textcolor{black}{56.12} & \textcolor{black}{2.26} & \textcolor{black}{1.80} & \textcolor{black}{1.67} \\
        Conformer-4 &  6.22M  &  \ding{52}   & \textcolor{black}{2.67} & \textcolor{black}{1.94} & \textcolor{black}{72.78} & \textcolor{black}{3.30} & \textcolor{black}{2.46} & \textcolor{black}{2.59}  \\
        Mamba-13   &  5.83M  &  \ding{52}   & \textcolor{black}{\bf 2.70} & \textcolor{black}{\bf 1.97} & \textcolor{black}{\bf 73.53} & \textcolor{black}{\bf 3.32} & \textcolor{black}{\bf 2.50} & \textcolor{black}{\bf 2.62}  \\
        \hdashline
        Conformer-4 & 6.22M  & \ding{55} & \textcolor{black}{2.88} & \textcolor{black}{2.17} & \textcolor{black}{76.68} & \textcolor{black}{3.51} & \textcolor{black}{2.61} & \textcolor{black}{2.82}  \\
        ExtBiMamba-6  &  5.39M  & \ding{55} & 2.88 & 2.18 & 76.73 & 3.50 & 2.62 & 2.82  \\
        ExtBiMamba-7  &  6.26M  & \ding{55} & \bf 2.90 & \bf 2.20 & \bf 77.04 & \bf 3.54 & \bf 2.64 & \bf 2.84  \\
        \hline
        \hline
        Conformer-6 &  9.26M  &  \ding{52}   & \textcolor{black}{2.68} & \textcolor{black}{1.94} & \textcolor{black}{73.41} & \textcolor{black}{3.30} & \textcolor{black}{2.46} & \textcolor{black}{2.59}  \\
        Mamba-20   &  8.89M  &  \ding{52}   & \textcolor{black}{\bf 2.72} & \textcolor{black}{\bf 2.00} & \textcolor{black}{\bf 74.09} & \textcolor{black}{\bf 3.35} & \textcolor{black}{\bf 2.51} & \textcolor{black}{\bf 2.65}  \\
        \hdashline
        Conformer-6 & 9.26M  & \ding{55} & \textcolor{black}{\bf 2.91} & \textcolor{black}{\bf 2.20} & \textcolor{black}{ 77.56} & \textcolor{black}{3.54} & \textcolor{black}{2.62} & \textcolor{black}{2.84}  \\
        ExtBiMamba-10  & 8.89M  & \ding{55} & \bf 2.91 & \bf 2.20 & \bf 77.64 & \bf 3.59 & \bf 2.65 & \bf 2.87 \\
        \toprule[1.0pt]
    \end{tabular}
    }
\end{table}


==> SE_table/Transformertime.tex <==
\begin{table}[t]
    \centering
    \scriptsize
    \def\arraystretch{1.25}
    \setlength{\tabcolsep}{1pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
    \caption{Training speed and inference speed of \textcolor{black}{ExtBiMamba} and non-causal Transformers.}
    \label{tab:transformertime}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lccc||ccc@{}}
        \toprule[1.0pt]
           & Transformer-4  & \textcolor{black}{ExtBiMamba-3} & \textcolor{black}{ExtBiMamba-4} & Transformer-6 & \textcolor{black}{ExtBiMamba-5} & \textcolor{black}{ExtBiMamba-6} \\
          \hline
          sec/step & 0.099  & 0.089 & 0.102 & 0.125 &  0.122 & 0.141 \\
          RTF(10s) & $1.48\times 10^{-4}$ & $1.08\times 10^{-4}$ & $1.38\times 10^{-4}$ &  $2.12\times 10^{-4}$  & $1.71\times 10^{-4}$ & $2.04\times 10^{-4}$ \\
          % RTF ($\times 10^{-4}$) & $1.48$ & $1.08$ & $1.38$ & $2.12$ & $1.71$ & $2.04$ \\
          RTF(40s) & $3.94\times 10^{-4}$ & $6.95\times 10^{-5}$ & $9.14\times 10^{-5}$ &  $5.89\times 10^{-4}$  & $1.13\times 10^{-4}$ & $1.35\times 10^{-4}$ \\
        \toprule[1.0pt]
    \end{tabular}
    }
\end{table}


==> SE_table/longer_speech.tex <==
\begin{table}[ht]
    \centering
    \scriptsize
    \def\arraystretch{1.02}
    \setlength{\tabcolsep}{1pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt}
    \setlength\aboverulesep{0pt}
    \setlength\belowrulesep{0pt}
    \caption{\textcolor{red}{Inference} speed comparison of Transformer and ExtBiMamba models \textcolor{blue}{for different input lengths.}}
    \label{tab:speed_comparison}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lcccccc@{}}
        \toprule[1.25pt]
           & Transformer-4  & \textcolor{black}{ExtBiMamba-3} & \textcolor{black}{ExtBiMamba-4} & Transformer-6 & \textcolor{black}{ExtBiMamba-5} & \textcolor{black}{ExtBiMamba-6} \\
          \hline
          sec/step & 0.099 & 0.089 & 0.102 & 0.125 & 0.122 & 0.141 \\
          RTF (10s) & $1.48 \times 10^{-4}$ & $1.08 \times 10^{-4}$ & $1.38 \times 10^{-4}$ & $2.12 \times 10^{-4}$ & $1.71 \times 10^{-4}$ & $2.04 \times 10^{-4}$ \\
          RTF (40s) & $3.94 \times 10^{-4}$ & $6.95 \times 10^{-5}$ & $9.14 \times 10^{-5}$ & $5.89 \times 10^{-4}$ & $1.13 \times 10^{-4}$ & $1.35 \times 10^{-4}$ \\
        \toprule[1.5pt]
    \end{tabular}
    }
    \label{longer Speech}
    \vspace{-1.25em}
\end{table}

==> SE_table/training_time.tex <==
\begin{table}[ht]
    \centering
    \scriptsize
    \def\arraystretch{1.02}
    \setlength{\tabcolsep}{1pt}
    \setlength{\abovetopsep}{0pt}
    \setlength\belowbottomsep{0pt} 
    \setlength\aboverulesep{0pt} 
    \setlength\belowrulesep{0pt}
    \caption{Training speed and inference speed of \textcolor{black}{ExtBiMamba} and non-causal Conformers.}
    \label{tab:conformertime}
    \resizebox{\columnwidth}{!}{
    \begin{tabular}{@{}lccc||cc@{}}
        \toprule[1.0pt]
           & Conformer-4  & \textcolor{black}{ExtBiMamba-6} & \textcolor{black}{ExtBiMamba-7} & Conformer-6 & \textcolor{black}{ExtBiMamba-10} \\
          \hline
          sec/step & 0.160 & 0.142 & 0.156 & 0.215 & 0.206 \\
          RTF & $2.27\times 10^{-4}$ & $2.07\times 10^{-4}$ & $2.37\times 10^{-4}$ &  $3.27\times 10^{-4}$  & $3.32\times 10^{-4}$  \\
        \toprule[1.0pt]
    \end{tabular}
    }
    % \vspace{-1.25em}
\end{table}

